Automated Statistical Model Discovery with Language Models

Statistical model discovery is a challenging search over a vast space of models subject to domain-specific constraints. Efficiently searching over this space requires expertise in modeling and the problem domain. Motivated by the domain knowledge and programming capabilities of large language models (LMs), we introduce a method for language model driven automated statistical model discovery. We cast our automated procedure within the principled framework of Box's Loop: the LM iterates between proposing statistical models represented as probabilistic programs, acting as a modeler, and critiquing those models, acting as a domain expert. By leveraging LMs, we do not have to define a domain-specific language of models or design a handcrafted search procedure, which are key restrictions of previous systems. We evaluate our method in three settings in probabilistic modeling: searching within a restricted space of models, searching over an open-ended space, and improving expert models under natural language constraints (e.g., this model should be interpretable to an ecologist). Our method identifies models on par with human expert designed models and extends classic models in interpretable ways. Our results highlight the promise of LM-driven model discovery.

==> figures_tex/improvement_deux.tex <==
\begin{figure}[ht] 
\label{fig:lotka_volterra_1}
\centering
\includegraphics[width=0.30\textwidth]{figures/stan_improve.pdf} 
\includegraphics[width=0.30\textwidth]{figures/lotka_improve.pdf} 
\caption{\textbf{Round-to-round improvement.} Model revision leads to improvements on average; improvement is not necessarily monotonic for a given dataset and run.
LOO score vs round for Stan experiments. We normalize the scores across programs proposed for 3 rounds of Box's Loop and average across datasets for the no metadata condition. 
Larger is better and error bars correspond to standard error. 
\textbf{(right)} Squared error vs round for Lotka-Volterra experiment. We report the squared error averaged across three different runs, for the warm-start, no constraint condition; smaller is better.
\label{fig:improvement}}
\end{figure}

==> figures_tex/lotka_volterra/lotka_code2.tex <==
\begin{figure*}[ht!]
\centering
\begin{tcolorbox}[
title={LM proposed Lotka-Volterra programs}]
\fontsize{7pt}{7pt}\selectfont
\ttfamily
\begin{lstlisting}[language=Python]
def no_warm_start(t, y, _coeffs):
  # Hypothesis 1: Logistic growth for prey with carrying capacity kappa
  # Hypothesis 2: Saturation effect in predation rate with parameter psi
  db_dt = alpha * b * (1 - b / kappa) - beta * b * c / (1 + psi * b)
  dc_dt = -gamma * c + delta * b * c - epsilon * c**2
\end{lstlisting}

\begin{lstlisting}[language=Python]
def warm_start_constrained(t, y, _mlp):
  inputs = jnp.array([b])  # Input is prey density (bunny population)
  # Neural network learns a modifier for the handling time based on prey density
  handling_time_modifier = _mlp(inputs)
  # Modulate the predation rate beta in a non-linear manner according to handling time
  db_dt = alpha * b - beta * b * c / (1 + handling_time_modifier[0] * b)
  dc_dt = -gamma * c + delta * b * c / (1 + handling_time_modifier[0] * b)
\end{lstlisting}

\begin{lstlisting}[language=Python]
def warm_start_unconstrained(t, y, _mlp):
  inputs = jfu.ravel_pytree((b, c))[0]
  mlp_output = _mlp(inputs)
  # Fine-tuned scaling of the MLP output to match the amplitude of data more closely
  db_dt = alpha * b - beta * b * c + 0.02 * mlp_output[0] # Reduced scaling for bunnies
  dc_dt = -gamma * c + delta * b * c + 0.06 * mlp_output[1] # Increased scaling for cats
\end{lstlisting}

\end{tcolorbox}
\caption{\textbf{LM can propose corrections to ODEs} \textbf{(top)} In the no warm-start variation, the LM introduces corrections informed by knowledge of predator-prey models (carrying capacity, predation saturation)
\textbf{(middle)} 
When prompted to introduce neural networks in an interpretable way, LM proposes to make the 
handling time parameter depend non-linearly on the prey density, extending the Holling's type II response, a traditional approach to modeling predation saturation. 
\textbf{(bottom)} 
When prompted to introduce neural networks without constraints, LM introduces additive MLP parameterized corrections and adjusts the scaling factors. 
}
\label{code:lotka-volterra_supp}


\end{figure*}




==> figures_tex/stan/stan_normal.tex <==
\begin{figure*}[t!]
    \includegraphics[width=0.35\textwidth]{figures/stan/eight_schools.png}
    \includegraphics[width=0.35\textwidth]{figures/stan/dugongs_data.png} 
    \includegraphics[width=0.35\textwidth]{figures/stan/GLM_Poisson_Data.png}
    \includegraphics[width=0.35\textwidth]{figures/stan/surgical_data.png}
    \caption{\textbf{Comparison of language model programs and expert programs on Stan PosteriorDB datasets} Language models identify programs on par or better than expert programs in terms of predictive accuracy.}
    \label{fig:natural}
\end{figure*}

==> figures_tex/stan/stan_simulated.tex <==
\begin{figure*}[t!]
    \includegraphics[width=0.35\textwidth]{figures/stan/eight_schools_simulated.png}
    \includegraphics[width=0.35\textwidth]{figures/stan/eight_schools_simulated_corrupt.png}    
 \includegraphics[width=0.35\textwidth]{figures/stan/dugongs_simulated.png} 
\includegraphics[width=0.35\textwidth]{figures/stan/dugongs_simulated_corrupt.png}     
\caption{Stan PosteriorDB simulated and corrupted ablation; LM program vs ground truth program}    \label{fig:simulated}
\end{figure*}

==> sections/background.tex <==
\subsection{Background}
\label{sec:background}
Before introducing our method, we provide a brief overview of the probabilistic modeling paradigm.
We then motivate a key design choice: representing probabilistic models with probabilistic programs. 
In probabilistic modeling, our goal is to describe a dataset in terms of unobserved, latent structure. 
Formally, a probabilistic model is a joint distribution $p(x, z| \eta);$ where $x=x_{1:N}$ denotes $N$ observed data points, $z = z_{1:M}$ denotes $M$ latent variables, and $\eta$ corresponds to non-random quantities in the model \citep{blei_build}.
After specifying a probabilistic model, we fit the model to observed data.
Fitting a model involves \textit{inference}, or computing the \textit{posterior distribution} $p(z|x)$.
In the model criticism step, we evaluate the model by interrogating the posterior. 
In this work, we use a common model criticism technique known as a \textit{posterior predictive check}: to identify discrepancies, we sample from the posterior predictive distribution and compare these samples against observed data \citep{Gelman2013BayesianDA}.
Model building and model criticism typically take place over multiple iterations in a process known as \textit{Box's Loop} \citep{Box1962AUM}.

There are many different representations of a probabilistic model. 
Since our goal is automated model discovery, we use \textit{probabilistic programs}.
Probabilistic programming languages provide ways to flexibly represent probabilistic models as programs and support generic inference methods for any arbitrary program \citep{wood-aistats-2014, Goodman2008ChurchAL, vandemeent2021introduction}. 
In the context of automated model discovery, these are highly desirable properties, since LMs can write code reliably and other representations of probabilistic models can require custom inference methods.
Our approach of using LMs to generate probabilistic programs is related to the approach taken by \citet{Wong2023FromWM} but is motivated by a different problem. 
Our emphasis is on using LMs as a tool for developing statistical models of real-world datasets, while their focus was on integrating symbolic methods with LMs to enhance their reasoning capabilities. 
\label{method}


==> table_tex/ablations.tex <==
\begin{tabular}{lrll}
\toprule
 corrupt &  exemplars &    loo &   waic \\
\midrule
   False &              1 & -16.81 & -14.02 \\
   False &              2 & -17.93 & -15.79 \\
   False &              3 & -16.83 & -13.82 \\
   False &              4 & -18.31 & -15.88 \\
    True &              1 & -18.11 & -15.80 \\
    True &              2 & -16.97 & -14.31 \\
    True &              3 & -16.36 & -13.92 \\
    True &              4 & -18.00 & -15.70 \\
\bottomrule
\end{tabular}

